Software Development Analytics in Practice: A Systematic Literature Review

Context:Software Development Analytics is a research area concerned with providing insights to improve product deliveries and processes. Many types of studies, data sources and mining methods have been used for that purpose. Objective:This systematic literature review aims at providing an aggregate view of the relevant studies on Software Development Analytics in the past decade, with an emphasis on its application in practical settings. Method:Definition and execution of a search string upon several digital libraries, followed by a quality assessment criteria to identify the most relevant papers. On those, we extracted a set of characteristics (study type, data source, study perspective, development life-cycle activities covered, stakeholders, mining methods, and analytics scope) and classified their impact against a taxonomy. Results:Source code repositories, experimental case studies, and developers are the most common data sources, study types, and stakeholders, respectively. Product and project managers are also often present, but less than expected. Mining methods are evolving rapidly and that is reflected in the long list identified. Descriptive statistics are the most usual method followed by correlation analysis. Being software development an important process in every organization, it was unexpected to find that process mining was present in only one study. Most contributions to the software development life cycle were given in the quality dimension. Time management and costs control were lightly debated. The analysis of security aspects suggests it is an increasing topic of concern for practitioners. Risk management contributions are scarce. Conclusions:There is a wide improvement margin for software development analytics in practice. For instance, mining and analyzing the activities performed by software developers in their actual workbench, the IDE.

==> chapter2-SumCost.tex <==
\textbf{Absent} & 29 & 69.05\% & [S03], [S05], [S06], [S07], [S09], [S10], [S12], [S13], [S14], [S15], [S16], [S17], [S18], [S19], [S20], [S22], [S23], [S24], [S25], [S26], [S27], [S28], [S29], [S30], [S31], [S32], [S33], [S41], [S42]\\[0.1cm]
\textbf{Weak} & 9 & 21.43\% & [S01], [S02], [S04], [S08], [S11], [S21], [S38], [S39], [S40]\\[0.1cm]
\textbf{Moderate} & 4 & 9.52\% & [S34], [S35], [S36], [S37]\\[0.1cm]
\hline


==> chapter2-SumDebt.tex <==
\textbf{Strong} & 28 & 66.67\% & [S01], [S02], [S04], [S05], [S06], [S07], [S08], [S09], [S10], [S11], [S12], [S13], [S14], [S15], [S16], [S17], [S18], [S19], [S20], [S24], [S25], [S30], [S32], [S36], [S37], [S39], [S40], [S41]\\[0.1cm]
\textbf{Moderate} & 9 & 21.43\% & [S03], [S22], [S23], [S26], [S28], [S31], [S35], [S38], [S42]\\[0.1cm]
\textbf{Weak} & 5 & 11.9\% & [S21], [S27], [S29], [S33], [S34]\\[0.1cm]
\hline


==> chapter2-SumPerspectives.tex <==
1 & \textbf{Post-Mortem} & 41 & 97.62\% & [S01], [S02], [S03], [S04], [S05], [S06], [S07], [S08], [S09], [S10], [S11], [S12], [S13], [S14], [S15], [S16], [S17], [S18], [S19], [S20], [S21], [S22], [S23], [S24], [S25], [S26], [S27], [S28], [S29], [S30], [S31], [S32], [S33], [S34], [S36], [S37], [S38], [S39], [S40], [S41], [S42]\\[0.2cm]
2 & \textbf{Pre-Mortem} & 1 & 2.38\% & [S35]\\[0.2cm]


==> chapter2-SumRisk.tex <==
\textbf{Absent} & 38 & 90.48\% & [S02], [S03], [S04], [S05], [S06], [S07], [S08], [S09], [S10], [S11], [S12], [S13], [S14], [S15], [S16], [S17], [S18], [S19], [S20], [S21], [S22], [S23], [S24], [S25], [S26], [S27], [S28], [S29], [S30], [S31], [S32], [S33], [S34], [S38], [S39], [S40], [S41], [S42]\\[0.1cm]
\textbf{Weak} & 4 & 9.52\% & [S01], [S35], [S36], [S37]\\[0.1cm]
\hline


==> chapter2-SumSecurity.tex <==
\textbf{Absent} & 37 & 88.1\% & [S02], [S03], [S04], [S05], [S06], [S07], [S08], [S09], [S10], [S11], [S12], [S13], [S14], [S15], [S16], [S17], [S18], [S19], [S20], [S21], [S22], [S23], [S24], [S25], [S26], [S28], [S31], [S32], [S33], [S34], [S35], [S37], [S38], [S39], [S40], [S41], [S42]\\[0.1cm]
\textbf{Moderate} & 2 & 4.76\% & [S27], [S29]\\[0.1cm]
\textbf{Weak} & 2 & 4.76\% & [S30], [S36]\\[0.1cm]
\textbf{Strong} & 1 & 2.38\% & [S01]\\[0.1cm]
\hline

==> chapter2-SumSources2.tex <==
%10 & 
\textbf{Android Issue Tracker} & 1 & 3.12\% & [S27]\\
%11 & 
\textbf{Apache OpenOffice Issue Tracking System} & 1 & 3.12\% & [S18]\\
%12 & 
\textbf{Apache Tomcat Archive} & 1 & 3.12\% & [S01]\\
%13 & 
\textbf{BinTray} & 1 & 3.12\% & [S09]\\
%14 & 
\textbf{Chrome Releases Blog} & 1 & 3.12\% & [S27]\\
%15 & 
\textbf{Chromium Issue Tracker} & 1 & 3.12\% & [S27]\\
%16 & 
\textbf{Exception Reports} & 1 & 3.12\% & [S07]\\
%17 & 
\textbf{Gerrit} & 1 & 3.12\% & [S11]\\
%18 & 
\textbf{Google} & 1 & 3.12\% & [S09]\\
%19 & 
\textbf{Google Forms} & 1 & 3.12\% & [S13]\\
%20 & 
\textbf{HackerOne Bug Bounty Platform} & 1 & 3.12\% & [S27]\\
%21 & 
\textbf{JCenter} & 1 & 3.12\% & [S09]\\
%22 & 
\textbf{JIRA} & 1 & 3.12\% & [S14]\\
%23 & 
\textbf{Lab Computers} & 1 & 3.12\% & [S15]\\
%24 & 
\textbf{Mailing List} & 1 & 3.12\% & [S26]\\
%25 & 
\textbf{Mercurial Repositories} & 1 & 3.12\% & [S16]\\
%26 & 
\textbf{NetBeans Source Code Repository} & 1 & 3.12\% & [S07]\\
%27 & 
\textbf{SecuriBench Archive} & 1 & 3.12\% & [S01]\\
%28 & 
\textbf{SEnerCON Feedback Gathering System} & 1 & 3.12\% & [S18]\\
%29 & 
\textbf{Team Wiki (BitBucket)} & 1 & 3.12\% & [S16]\\
%30 & 
\textbf{Version Control Repositories} & 1 & 3.12\% & [S25]\\
%31 & 
\textbf{Vulnerability Reports} & 1 & 3.12\% & [S01]\\



==> chapter2-SumTime.tex <==
\textbf{Absent} & 23 & 54.76\% & [S03], [S04], [S05], [S06], [S07], [S09], [S10], [S12], [S13], [S14], [S16], [S17], [S20], [S22], [S24], [S25], [S27], [S28], [S29], [S31], [S32], [S33], [S42]\\[0.1cm]
\textbf{Moderate} & 11 & 26.19\% & [S15], [S21], [S26], [S34], [S35], [S36], [S37], [S38], [S39], [S40], [S41]\\[0.1cm]
\textbf{Weak} & 8 & 19.05\% & [S01], [S02], [S08], [S11], [S18], [S19], [S23], [S30]\\[0.1cm]
\hline

==> chapter2-articles_no_score.tex <==
\textbf{S01} & 2019 & Sultana et al. & A study examining relationships between micro patterns and security vulnerabilities & Software Quality Journal \\[0.1cm]
\textbf{S02} & 2019 & Jha et al. & An empirical study of configuration changes and adoption in Android apps & Journal of Systems and Software \\[0.1cm]
\textbf{S03} & 2017 & Hassan et al. & An empirical study of emergency updates for top android mobile apps & Empirical Software Engineering \\[0.1cm]
\textbf{S04} & 2016 & W. Wu et al. & An exploratory study of api changes and usages based on apache and eclipse ecosystems & Empirical Software Engineering \\[0.1cm]
\textbf{S05} & 2017 & Taba et al. & An exploratory study on the usage of common interface elements in android applications & Journal of Systems and Software \\[0.1cm]
\textbf{S06} & 2019 & Prana et al. & Categorizing the Content of GitHub README Files & Empirical Software Engineering \\[0.1cm]
\textbf{S07} & 2018 & R. Wu et al. & ChangeLocator: locate crash-inducing changes based on crash reports & Empirical Software Engineering \\[0.1cm]
\textbf{S08} & 2019 & Yan et al. & Characterizing and identifying reverted commits & Empirical Software Engineering \\[0.1cm]
\textbf{S09} & 2018 & Salza et al. & Do developers update third-party libraries in mobile apps? & Proceedings of the International Conference on Program Comprehension \\[0.1cm]
\textbf{S10} & 2019 & Liu et al. & DroidLeaks: a comprehensive database of resource leaks in Android apps & Empirical Software Engineering \\[0.1cm]
\textbf{S11} & 2018 & Fan et al. & Early prediction of merged code changes to prioritize reviewing tasks & Empirical Software Engineering \\[0.1cm]
\textbf{S12} & 2016 & McIlroy et al. & Fresh apps: an empirical study of frequently-updated mobile apps in the Google play store & Empirical Software Engineering \\[0.1cm]
\textbf{S13} & 2018 & Saborido et al. & Getting the most from map data structures in Android & Empirical Software Engineering \\[0.1cm]
\textbf{S14} & 2017 & Guerrouj et al. & Investigating the relation between lexical smells and change- and fault-proneness: an empirical study & Software Quality Journal \\[0.1cm]
\textbf{S15} & 2014 & Fucci et al. & On the role of tests in test-driven development: a differentiated and partial replication & Empirical Software Engineering \\[0.1cm]
\textbf{S16} & 2014 & Mittal et al. & Process mining software repositories from student projects in an undergraduate software engineering course & Proceedings of the International Conference on Software Engineering \\[0.1cm]
\textbf{S17} & 2018 & Rakha et al. & Revisiting the performance of automated approaches for the retrieval of duplicate reports in issue tracking systems that perform just-in-time duplicate retrieval & Empirical Software Engineering \\[0.1cm]
\textbf{S18} & 2018 & Morales-Ramirez et al. & Speech-acts based analysis for requirements discovery from online discussions & Information Systems Journal \\[0.1cm]
\textbf{S19} & 2018 & Li et al. & Studying software logging using topic models & Empirical Software Engineering \\[0.1cm]
\textbf{S20} & 2018 & Hassan et al. & Studying the dialogue between users and developers of free apps in the Google Play Store & Empirical Software Engineering \\[0.1cm]
\textbf{S21} & 2016 & Rakha et al. & Studying the needed effort for identifying duplicate issues & Empirical Software Engineering \\[0.1cm]
\textbf{S22} & 2017 & Ye et al. & The structure and dynamics of knowledge network in domain-specific Q\&A sites: a case study of stack overflow & Empirical Software Engineering \\[0.1cm]
\textbf{S23} & 2019 & Sawant et al. & To react, or not to react: Patterns of reaction to API deprecation & Empirical Software Engineering \\[0.1cm]
\textbf{S24} & 2019 & Cruz et al. & To the attention of mobile software developers: guess what, test your app! & Empirical Software Engineering \\[0.1cm]
\textbf{S25} & 2017 & Li et al. & Towards just-in-time suggestions for log changes & Empirical Software Engineering \\[0.1cm]
\textbf{S26} & 2017 & Izquierdo-Cortazar et al. & Using Metrics to track code review performance & International Conference on Evaluation and Assessment in Software Engineering \\[0.1cm]
\textbf{S27} & 2016 & Munaiah et al. & Vulnerability severity scoring and bounties: Why the disconnect? & Proceedings of the International Workshop on Software Analytics \\[0.1cm]
\textbf{S28} & 2015 & Tian et al. & What are the characteristics of high-rated apps? A case study on free Android Applications & Proceedings of the International Conference on Software Maintenance and Evolution \\[0.1cm]
\textbf{S29} & 2016 & Yang et al. & What security questions do developers ask? a large-scale study of stack overflow posts & Journal of Computer Science and Technology \\[0.1cm]
\textbf{S30} & 2019 & Chen et al. & What's Spain's Paris ? Mining analogical libraries from Q\&A discussions & Empirical Software Engineering \\[0.1cm]
\textbf{S31} & 2017 & Jiang et al. & Why and how developers fork what from whom in GitHub & Empirical Software Engineering \\[0.1cm]
\textbf{S32} & 2019 & Thongtanunam et al. & Will this clone be short-lived? Towards a better understanding of the characteristics of short-lived clones & Empirical Software Engineering \\[0.1cm]


==> chapter2-graphics.tex <==
\plot{chapter2-1.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-10.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-11.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-12.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-13.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-14.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-15.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-16.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-17.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-18.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-19.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-2.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-20.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-21.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-22.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-23.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-3.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-30.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-35.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-36.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-37.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-4.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-40.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-5.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-6.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-7.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-8.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]
\plot{chapter2-9.pdf}[Put Your Caption Here][12][H][trim=0cm 0cm 0cm 0cm]


==> continents.tex <==
\begin{comment}

\begin{table}[!htbp]
\caption{Statistics per Continent}
\label{table:SumContinents}
\centering
\begin{tabular}{p{2.7cm}ccp{5.8cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#
	\textbf{Country} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

   \input{chapter2-SumContinents}


   \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\end{comment}


%{\renewcommand{\arraystretch}{1.8}
\begin{longtable}{p{2.7cm}ccp{5.8cm}}
   \caption{Statistics per Continent}
\label{table:SumContinents}
    \\\hline\noalign{\smallskip}
	%\textbf{\#} & 
		\textbf{Name} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
    \noalign{\smallskip}\hline\noalign{\smallskip}
\endfirsthead


\multicolumn{4}{c}
%{ \tablename\ \thetable{}: continued from previous page } \\ 
{ \begin{footnotesize} \tablename\ \thetable{}: continued from previous page \end{footnotesize} } \\


\hline\noalign{\smallskip}

   	%\textbf{\#} & 
   		\textbf{Name} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\

\noalign{\smallskip}\hline\noalign{\smallskip}
\endhead

\hline \multicolumn{4}{r}{{Continued on next page}} \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\endfoot
 

\hline
\endlastfoot

    \input{chapter2-SumContinents}

\noalign{\smallskip}\hline
%\multicolumn{4}{l}{\shortstack[l]{\textbf{Freq.} - Frequency, \textbf{Perc.} - Percentage, \textbf{Ref.} - Reference}}
\end{longtable}




==> costs.tex <==
\begin{table*}[ht]
\caption{Costs Control}
\label{table:CostsControl}
\centering
\begin{tabular}{p{1.3cm}ccp{6.5cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Benefit} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{chapter2-SumCost}

   \noalign{\smallskip}\hline
\end{tabular}
\end{table*}

==> countries.tex <==
\begin{comment}

\begin{table}[H]
\caption{Statistics per Country}
\label{table:SumCountries}
\centering
\begin{tabular}{p{3.2cm}ccp{5cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#
	\textbf{Country} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

   \input{chapter2-SumCountries}


   \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\end{comment}


%{\renewcommand{\arraystretch}{1.8}
\begin{longtable}{p{3.2cm}ccp{5cm}}
    \caption{Statistics per Country}
\label{table:SumCountries}
    \\\hline\noalign{\smallskip}
	%\textbf{\#} & 
		\textbf{Name} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
    \noalign{\smallskip}\hline\noalign{\smallskip}
\endfirsthead


\multicolumn{4}{c}
%{ \tablename\ \thetable{}: continued from previous page } \\ 
{ \begin{footnotesize} \tablename\ \thetable{}: continued from previous page \end{footnotesize} } \\


\hline\noalign{\smallskip}

   	%\textbf{\#} & 
   		\textbf{Name} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\

\noalign{\smallskip}\hline\noalign{\smallskip}
\endhead

\hline \multicolumn{4}{r}{{Continued on next page}} \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\endfoot
 

\hline
\endlastfoot

    \input{chapter2-SumCountries}

\noalign{\smallskip}\hline
%\multicolumn{4}{l}{\shortstack[l]{\textbf{Freq.} - Frequency, \textbf{Perc.} - Percentage, \textbf{Ref.} - Reference}}
\end{longtable}



==> debt.tex <==
\begin{table*}[ht]
\caption{Technical Debt}
\label{table:TechnicalDebt}
\centering
\begin{tabular}{p{1.3cm}ccp{12cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Benefit} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{chapter2-SumDebt}


   %\noalign{\smallskip}\hline
\end{tabular}
\end{table*}

==> perspectives.tex <==
\begin{table}[!htbp]
\caption{Project/Process Perspective Findings}
\label{table:SumPerspectives}
\centering
\begin{tabular}{cp{2.35cm}ccp{3.65cm}}
	\hline\noalign{\smallskip}
	\textbf{\#} & \textbf{Perspective} & \textbf{Frequency} & \textbf{Percentage} & \textbf{Reference}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
 
 \input{chapter2-SumPerspectives}

   \noalign{\smallskip}\hline
\end{tabular}
\end{table}

==> risks.tex <==
\begin{table*}[!htbp]
\caption{Risks Assessment}
\label{table:RisksAssessment}
\centering
\begin{tabular}{p{1.3cm}ccp{12cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Benefit} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{chapter2-SumRisk}


  %\noalign{\smallskip}\hline
\end{tabular}
\end{table*}

==> security.tex <==
\begin{table*}[!htbp]
\caption{Security Analysis}
\label{table:SecurityAnalysis}
\centering
\begin{tabular}{p{1.3cm}ccp{12cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Benefit} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{chapter2-SumSecurity}


  %\noalign{\smallskip}\hline
\end{tabular}
\end{table*}

==> sources2.tex <==

\begin{comment}

\footnotesize

\begin{table}[!htbp]
\caption{Data Sources Findings - Remaining (Frequency $=$ 1)}
\label{table:SumSources2}
\centering
\begin{tabular}{p{4cm}ccp{1.8cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Data Sources} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}
 
 \input{chapter2-SumSources2}


   \noalign{\smallskip}\hline
\end{tabular}
\end{table}

\normalsize

\end{comment}


%{\renewcommand{\arraystretch}{1.8}
\begin{longtable}{p{8cm}ccc}
    \caption{Data Sources Findings - Remaining (Frequency $=$ 1)}
    \label{table:SumSources2}
    \\\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Data Sources} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
    \noalign{\smallskip}\hline\noalign{\smallskip}
\endfirsthead


\multicolumn{4}{c}
%{ \tablename\ \thetable{}: continued from previous page } \\ 
{ \begin{footnotesize} \tablename\ \thetable{}: continued from previous page \end{footnotesize} } \\


\hline\noalign{\smallskip}

   	%\textbf{\#} & 
   	\textbf{Data Sources} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\

\noalign{\smallskip}\hline\noalign{\smallskip}
\endhead

\hline \multicolumn{4}{r}{{Continued on next page}} \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\endfoot

\hline
\endlastfoot

 \input{chapter2-SumSources2}

\noalign{\smallskip}\hline

\end{longtable}
%}



==> studies_analysis.tex <==
\textbf{S3}~\cite{Sultana2019AVulnerabilities} Various security models focus on different phases of the software development including requirement analysis phase, design phase, implementation phase, and testing phase to
ensure security. The existing metrics at the code or implementation level are basically software
metrics that are used for security assessment, and they have high false negative rates.

Limitation in the data sources: We address all research questions using the Apache Tomcat datasets. Research questions RQ1 and RQ4 are evaluated using our secondary dataset, the Stanford SecuriBench, which
did not contain information across development versions needed to address questions RQ2
and RQ3.

Most of the existing literature focuses on complexity metrics for software
quality assessment. Researchers have found that complexity is related with software faults
and other problematic issues (Shin 2008). Researchers also determined that the fault prediction
models based on complexity metrics might be useful for vulnerability prediction, and
some metrics, such as nesting complexity metrics, are more effective for locating vulnerable
code than locating faulty code (Shin and Williams 2008b). Shin et al. (2008a, 2013)
conducted an empirical study to analyze the impacts of complexity metrics on vulnerable
and non-vulnerable files.



\textbf{S14}~\cite{Yan2019CharacterizingCommits}
In addition, we found that “developer” is
the most discriminative dimension among the three dimensions of features for the identification
of reverted commits. However, using all the three dimensions of commit features
leads to better performance.
Using our tool, possibly reverted commits
can be detected in an early stage. Then, developers can fix them or revert them early.
Third, there are some common important features in our studied projects, such the developer
related features “EXP” and “NDEV”. It means that developers should pay more attention
to the commits made by non-expert developers of the project.


\textbf{S16}~\cite{SalzaDoApps}
Developers rarely update third-party libraries
in mobile apps, i.e., only 2 % of commits. When an update is
performed, it is usually an upgrade toward a newer version.
However, in some cases developers prefer to downgrade because
of the issues caused by a previous upgrade.

Third-party libraries related to the graphical user
interface or providing support tools for development are the
ones having the highest number of version changes in the mobile
apps using them. This is mainly due to the will of developers
to (1) keep the GUI always up to date with the latest graphical
tendencies, or (2) update Android support tools to support the
latest Android versions.

Developers followpeculiar update patterns when
dealing with library updates. Only in 13 % of the cases the used
external libraries are constantly updated by developers, while
we found that in 63 % of the cases external library uses are never
updated after their introduction.


\textbf{S18}~\cite{Liu2019DroidLeaks:Apps}
This paper presented DROIDLEAKS, a database of 292 resource leak bugs in real-world
Android apps. We constructed DROIDLEAKS by analyzing 124,215 code revisions of 34
popular open-source app subjects. To understand the characteristics of these bugs, we conducted
an empirical study and discovered common resource management mistakes made by
developers. To show the usefulness of our study, we evaluated eight existing resource leak
detectors for Android apps using DROIDLEAKS. The evaluation led to a detailed analysis of
the limitations and strengths of the detectors.

\textbf{S19}~\cite{Fan2018EarlyTasks} 
Besides, we also study the important features which distinguish
merged code changes from abandoned ones.
In this paper, we propose an approach to predict whether a code change will be merged.We
extract 34 features to characterize a code change; these features are grouped into five dimensions:
code, file history, owner experience, collaboration network and text. We use random
forest to build a prediction model and use cost sensitive learning to deal with imbalanced
data.

\textbf{S20}~\cite{McIlroy2016FreshStore} 


==> time.tex <==
\begin{table*}[ht]
\caption{Time Management}
\label{table:TimeManagement}
\centering
\begin{tabular}{p{1.3cm}ccp{6.5cm}}
	\hline\noalign{\smallskip}
	%\textbf{\#} & 
	\textbf{Benefit} & \textbf{Freq.} & \textbf{Perc.} & \textbf{Ref.}\\
	\noalign{\smallskip}\hline\noalign{\smallskip}

 \input{chapter2-SumTime}


   \noalign{\smallskip}\hline
\end{tabular}
\end{table*}
